Political Openness and Armed Conflict: Evidence from Local Councils in Colombia

In this paper, I empirically investigate how the openness of political institutions to diverse representation can impact conflict-related violence. By exploiting plausibly exogenous variations in the number of councillors in Colombian municipalities, I develop two sets of results. First, regression discontinuity estimates show that larger municipal councils have a considerably greater number of political parties with at least one elected representative. I interpret this result as evidence that larger municipal councils are more open to diverse political participation. The estimates also reveal that non-traditional parties are the main beneficiaries of this greater political openness. Second, regression discontinuity estimates show that political openness substantially decreases conflict-related violence, namely the killing of civilian non-combatants. By exploiting plausibly exogenous variations in local election results, I show that the lower level of political violence stems from greater participation by parties with close links to armed groups. Using data about the types of violence employed by these groups, and representation at higher levels of government, I argue that armed violence has decreased not because of power-sharing arrangements involving armed groups linked to the parties with more political representation, but rather because armed groups with less political power and visibility are deterred from initiating certain types of violence.

==> TABLE_A18.tex <==
paramilitary-linked mayor&      -0.011         &      -0.007         &      -0.005\sym{**} &      -0.011         &      -0.006         &      -0.005\sym{**} \\
                    &     (0.008)         &     (0.007)         &     (0.002)         &     (0.008)         &     (0.007)         &     (0.002)         \\
R-sq                &       0.714         &       0.717         &       0.509         &       0.716         &       0.719         &       0.509         \\
Observations        &        1858         &        1858         &        1858         &        1852         &        1852         &        1852         \\


==> TABLE_A19_panelA.tex <==
RD Estimate &       0.052\sym{**} &       0.051\sym{**} &       0.003         &       0.098         &       0.062         \\
            &     (0.022)         &     (0.021)         &     (0.003)         &     (0.085)         &     (0.074)         \\
Observations&         385         &         385         &         385         &         347         &         347         \\
Eff. Number of obs&         260         &         260         &         247         &         174         &         222         \\
BW Loc. Poly. (h)&       0.167         &       0.167         &       0.155         &       0.117         &       0.158         \\
Robust p-value&       0.020         &       0.017         &       0.297         &       0.253         &       0.375         \\


==> TABLE_A19_panelB.tex <==
RD Estimate &       0.030         &       0.040         &      -0.005         &       0.131         &       0.054         \\
            &     (0.026)         &     (0.026)         &     (0.004)         &     (0.104)         &     (0.059)         \\
Observations&         385         &         385         &         385         &         347         &         347         \\
Eff. Number of obs&         214         &         196         &         214         &         172         &         203         \\
BW Loc. Poly. (h)&       0.125         &       0.118         &       0.126         &       0.115         &       0.144         \\
Robust p-value&       0.222         &       0.100         &       0.278         &       0.204         &       0.381         \\


==> TABLE_A22_panelA.tex <==
RD Estimate &       0.142         &      -0.054         &       0.011         \\
            &     (0.091)         &     (0.083)         &     (0.028)         \\
Observations&        1899         &        1899         &        1899         \\
Eff. Number of obs&         420         &         478         &         423         \\
BW Loc. Poly. (h)&       0.090         &       0.102         &       0.091         \\
Robust p-value&       0.228         &       0.571         &       0.786         \\


==> TABLE_A22_panelB.tex <==
RD Estimate &       0.007         &       0.002         &       0.025         \\
            &     (0.052)         &     (0.032)         &     (0.093)         \\
Observations&        1900         &        1900         &        1900         \\
Eff. Number of obs&         551         &         502         &         497         \\
BW Loc. Poly. (h)&       0.119         &       0.107         &       0.106         \\
Robust p-value&       0.840         &       0.992         &       0.986         \\


==> TABLE_A23_panelA.tex <==
RD Estimate &       0.775         &       1.313\sym{**} \\
            &     (0.649)         &     (0.512)         \\
Observations&         927         &         973         \\
Eff. Number of obs&         242         &         140         \\
BW Loc. Poly. (h)&       0.109         &       0.059         \\
Robust p-value&       0.351         &       0.010         \\


==> TABLE_A23_panelB.tex <==
RD Estimate &       0.461         &       1.276\sym{***}\\
            &     (0.652)         &     (0.495)         \\
Observations&         927         &         973         \\
Eff. Number of obs&         226         &         135         \\
BW Loc. Poly. (h)&       0.102         &       0.056         \\
Robust p-value&       0.623         &       0.009         \\


==> TABLE_A23_panelC.tex <==
RD Estimate &      -0.035         &      -0.077\sym{**} \\
            &     (0.032)         &     (0.032)         \\
Observations&         927         &         973         \\
Eff. Number of obs&         285         &         188         \\
BW Loc. Poly. (h)&       0.127         &       0.077         \\
Robust p-value&       0.390         &       0.017         \\


==> TABLE_A7.tex <==
RD Estimate &       0.816\sym{*}  \\
            &     (0.417)         \\
Observations&        1900         \\
Eff. Number of obs&         390         \\
BW Loc. Poly. (h)&       0.082         \\
Robust p-value&       0.070         \\


==> arxiv last/TABLE_1.tex <==
\midrule
0-5000      &           7&          62&          91&         125&         152&         178&         211\\
5001-10000  &           9&         104&         126&         231&         243&         350&         351\\
10001-20000 &          11&          84&          91&         197&         174&         322&         268\\
20001-50000 &          13&          40&          34&          79&          64&         121&          89\\
50001-100000&          15&          20&          15&          35&          26&          50&          40\\
100001-250000&          17&           2&           7&           9&          12&          14&          18\\
250001-1000000&          19&           1&           0&           2&           0&           4&           2\\


==> arxiv last/TABLE_10.tex <==
RD Estimate &       0.023         &      -0.041         &       0.085         &       0.082         &       0.134         &      -0.010         \\
            &     (0.105)         &     (0.085)         &     (0.162)         &     (0.079)         &     (0.557)         &     (0.016)         \\
Observations&        2343         &        2341         &        2341         &        2341         &        1769         &        2344         \\
Eff. Number of obs&         575         &         517         &         501         &         674         &         396         &         378         \\
BW Loc. Poly. (h)&       0.097         &       0.088         &       0.084         &       0.114         &       0.091         &       0.064         \\
Robust p-value&       0.971         &       0.593         &       0.762         &       0.358         &       0.923         &       0.364         \\


==> arxiv last/TABLE_11_panelA.tex <==
RD Estimate &       0.112         &      -2.559\sym{*}  &       0.981         &       1.238         &      -2.149         \\
            &     (2.033)         &     (1.321)         &     (3.011)         &     (2.314)         &     (3.018)         \\
Observations&        2349         &        2349         &        2349         &        1189         &        1160         \\
Eff. Number of obs&         651         &         595         &         688         &         300         &         277         \\
BW Loc. Poly. (h)&       0.110         &       0.100         &       0.116         &       0.095         &       0.098         \\
Robust p-value&       0.901         &       0.038         &       0.532         &       0.439         &       0.491         \\


==> arxiv last/TABLE_11_panelB.tex <==
RD Estimate &       4.646         &      -2.731         &       0.565         &       6.990\sym{*}  &      -1.063         \\
            &     (3.835)         &     (1.911)         &     (3.755)         &     (4.031)         &     (5.210)         \\
Observations&        1016         &        1016         &        1016         &         498         &         518         \\
Eff. Number of obs&         271         &         235         &         253         &         111         &         137         \\
BW Loc. Poly. (h)&       0.118         &       0.100         &       0.109         &       0.103         &       0.111         \\
Robust p-value&       0.251         &       0.120         &       0.777         &       0.090         &       0.853         \\


==> arxiv last/TABLE_2.tex <==
            &         (1)&         (2)&         (3)&         (4)&         (5)&         (6)&         (7)&         (8)\\
\midrule
\emph{\textbf{Conflict-related violence (pre-election term)}}&            &            &            &            &            &            &            &            \\
Killings (overall)&        2355&       2.619&       6.646&         598&       2.229&       5.869&      -0.653&       0.545\\
Very selective killings&        2355&       1.746&       4.237&         598&       1.455&       3.665&      -0.499&       0.382\\
Massacres   &        2355&       0.873&       3.063&         598&       0.774&       2.654&      -0.246&       0.287\\
Occurrence of a killing (overall)&        2355&       0.076&       0.120&         598&       0.065&       0.109&      -0.018&       0.016\\
Occurrence of a very selective killing&        2355&       0.069&       0.112&         598&       0.059&       0.101&      -0.018&       0.015\\
Occurrence of a massacre&        2355&       0.011&       0.034&         598&       0.011&       0.032&      -0.002&       0.003\\
\emph{\textbf{Armed conflict (pre-election term)}}&            &            &            &            &            &            &            &            \\
Action by guerrilla&        1900&       0.480&       0.403&         468&       0.469&       0.402&      -0.075&       0.073\\
Action by paramilitaries&        1900&       0.206&       0.292&         468&       0.201&       0.277&      -0.046&       0.063\\
Action by Nal. army&        1900&       0.436&       0.385&         468&       0.442&       0.387&      -0.123&       0.071\\
Encounter paramilitaries vs guerrilla&        1900&       0.138&       0.256&         468&       0.122&       0.240&      -0.017&       0.058\\
Encounter Nal. army vs guerrilla&        1900&       0.363&       0.381&         468&       0.356&       0.379&      -0.086&       0.067\\
Encounter Nal. army vs paramilitaries&        1900&       0.116&       0.233&         468&       0.110&       0.218&      -0.011&       0.041\\
Event of massive expulsion&        2355&       0.085&       0.199&         598&       0.088&       0.210&      -0.057&       0.038\\
\emph{\textbf{Crime (pre-election term)}}&            &            &            &            &            &            &            &            \\
Overall homicide rate&        2315&      58.840&      56.840&         583&      58.897&      59.844&      -1.246&       8.074\\
Log of hectares of coca&        1931&       1.147&       2.294&         498&       1.244&       2.399&      -0.554&       0.456\\
Log of hectares of aerial spraying on coca&        1931&       0.745&       2.050&         498&       0.858&       2.164&      -0.663&       0.448\\
\emph{\textbf{Elections (previous election)}}&            &            &            &            &            &            &            &            \\
Turnout rate&        1423&       0.572&       0.105&         376&       0.578&       0.103&      -0.013&       0.020\\
Number of parties in council&        1905&       5.221&       2.110&         489&       5.327&       2.113&       0.643&       0.332\\
Council fractionalization&        2349&       0.975&       0.100&         596&       0.985&       0.078&      -0.017&       0.013\\
Liberal party in council&        1905&       0.898&       0.303&         489&       0.857&       0.351&       0.094&       0.050\\
Conservative party in council&        1905&       0.708&       0.455&         489&       0.681&       0.467&       0.175&       0.078\\
Left-wing party in council&        1905&       0.256&       0.437&         489&       0.254&       0.436&       0.017&       0.068\\
Party with paramilitary links in council&        1905&       0.510&       0.500&         489&       0.560&       0.497&       0.057&       0.078\\
Mayor from Liberal party&        2349&       0.359&       0.480&         596&       0.344&       0.475&      -0.041&       0.074\\
Mayor from Conservative party&        2349&       0.174&       0.379&         596&       0.181&       0.386&       0.081&       0.056\\
Mayor from left-wing party&        2349&       0.027&       0.162&         596&       0.020&       0.141&       0.022&       0.032\\
Mayor from party with paramilitary links&        2349&       0.076&       0.265&         596&       0.096&       0.294&       0.063&       0.048\\
\emph{\textbf{Economy and institutions}}&            &            &            &            &            &            &            &            \\
Municipal category (first year of term)&        1424&       5.396&       1.347&         377&       5.414&       1.271&       0.158&       0.186\\
\% unsatisfied basic needs (1993 or 2005)&        2355&      48.479&      22.310&         598&      48.100&      22.708&      -4.549&       2.964\\
Schools per 1000 inhab. (1997)&        2213&      34.779&      19.559&         554&      37.190&      20.639&      -3.234&       4.450\\
Hospitals per 1000 inhab. (1997)&        2213&       2.842&       2.561&         554&       2.941&       2.716&      -0.464&       0.387\\
Bank branches per 1000 inhab. in 1997&        2028&       7.364&       3.928&         502&       7.458&       3.756&       0.479&       0.690\\
Courts per 1000 inhab. (1997)&        2213&      10.030&       7.906&         555&      10.212&       8.190&       1.289&       1.384\\
Police stations per 1000 inhab. (1997)&        2208&       4.306&       2.123&         552&       4.432&       2.139&      -0.213&       0.274\\
\emph{\textbf{Fiscal outcomes (pre-election term)}}&            &            &            &            &            &            &            &            \\
Log current spending per capita&        2331&      -2.526&       0.537&         593&      -2.519&       0.557&       0.043&       0.094\\
Log fixed capital spending per capita&        2331&      -2.222&       0.630&         593&      -2.167&       0.674&       0.059&       0.117\\
Log other capital spending per capita&        2326&      -2.014&       0.932&         593&      -1.962&       0.903&       0.022&       0.165\\
Log tax revenue per capita&        2330&      -3.291&       1.153&         592&      -3.268&       1.156&       0.071&       0.170\\
Log royalties per capita&        1661&      -5.075&       2.591&         419&      -5.031&       2.665&       0.113&       0.596\\
Log transfers per capita&        2308&      -1.728&       0.546&         590&      -1.708&       0.542&       0.119&       0.084\\
Total deficit per capita&        2334&      -0.018&       0.234&         593&      -0.033&       0.414&      -0.066&       0.084\\
\emph{\textbf{Geographic characteristics}}&            &            &            &            &            &            &            &            \\
Surface area (km2)&        2355&    1223.097&    3634.450&         598&    1367.573&    4335.841&    -919.130&     658.769\\
Mean altitude (m)&        2294&     991.990&    1424.019&         576&     985.476&     918.371&     154.226&     141.588\\
Distance to Bogota (km)&        2355&     353.962&     192.983&         598&     354.501&     195.120&       1.050&      22.075\\
Distance to the capital of department (km)&        2355&      77.396&      60.821&         598&      75.774&      60.309&      -5.536&       9.593\\
\% Municipalities on the Atlantic coast&        2355&       0.248&       0.432&         598&       0.241&       0.428&       0.026&       0.095\\
\% Municipalities in the eastern region&        2355&       0.186&       0.390&         598&       0.224&       0.417&       0.071&       0.076\\
\% Municipalities in the central region&        2355&       0.172&       0.377&         598&       0.154&       0.361&       0.000&       0.060\\
\% Municipalities on the Pacific coast&        2355&       0.199&       0.399&         598&       0.197&       0.398&      -0.083&       0.067\\
\% Municipalities in Antioquia&        2355&       0.144&       0.352&         598&       0.129&       0.335&      -0.026&       0.068\\
\% Municipalities in the Amazon region&        2355&       0.050&       0.218&         598&       0.055&       0.229&       0.029&       0.037\\


==> arxiv last/TABLE_3.tex <==
RD Estimate &       0.158         &       0.133         &      -0.105         \\
            &     (0.186)         &     (0.173)         &     (0.161)         \\
Observations&        1424         &        1427         &        1427         \\
Eff. Number of obs&         444         &         377         &         429         \\
BW Loc. Poly. (h)&       0.118         &       0.100         &       0.115         \\
Robust p-value&       0.418         &       0.431         &       0.603         \\


==> arxiv last/TABLE_4.tex <==
RD Estimate &       0.028         &       0.314         &       1.108\sym{***}&       0.959\sym{**} \\
            &     (0.029)         &     (0.710)         &     (0.406)         &     (0.413)         \\
Observations&        1474         &        2355         &        2355         &        2355         \\
Eff. Number of obs&         367         &         494         &         514         &         479         \\
BW Loc. Poly. (h)&       0.099         &       0.082         &       0.086         &       0.080         \\
Robust p-value&       0.353         &       0.717         &       0.018         &       0.036         \\


==> arxiv last/TABLE_5_panelA.tex <==
RD Estimate &      -0.045\sym{***}&      -0.040\sym{**} &      -0.006         &       0.013         \\
            &     (0.016)         &     (0.016)         &     (0.004)         &     (0.022)         \\
Observations&        2355         &        2355         &        2355         &        2325         \\
Eff. Number of obs&         704         &         627         &         573         &         437         \\
BW Loc. Poly. (h)&       0.118         &       0.106         &       0.096         &       0.075         \\
Robust p-value&       0.011         &       0.017         &       0.190         &       0.400         \\


==> arxiv last/TABLE_5_panelB.tex <==
RD Estimate &      -1.099         &      -0.921\sym{*}  &      -0.126         &      -3.580         \\
            &     (0.712)         &     (0.471)         &     (0.291)         &     (4.078)         \\
Observations&        2355         &        2355         &        2355         &        2325         \\
Eff. Number of obs&         544         &         548         &         657         &         569         \\
BW Loc. Poly. (h)&       0.093         &       0.093         &       0.111         &       0.097         \\
Robust p-value&       0.134         &       0.071         &       0.637         &       0.471         \\


==> arxiv last/TABLE_5_panelC.tex <==
RD Estimate &      -2.829         &      -2.955\sym{*}  &      -0.010         &      -4.488         \\
            &     (2.408)         &     (1.744)         &     (0.982)         &     (9.656)         \\
Observations&        2355         &        2355         &        2355         &        2318         \\
Eff. Number of obs&         558         &         583         &         598         &         589         \\
BW Loc. Poly. (h)&       0.095         &       0.097         &       0.100         &       0.101         \\
Robust p-value&       0.292         &       0.097         &       0.936         &       0.696         \\


==> arxiv last/TABLE_6.tex <==
RD Estimate &       0.298\sym{***}&      -0.006         &      -0.064         &       0.196\sym{***}\\
            &     (0.071)         &     (0.072)         &     (0.045)         &     (0.066)         \\
Observations&        2355         &        2355         &        2355         &        2355         \\
Eff. Number of obs&         573         &         639         &         405         &         426         \\
BW Loc. Poly. (h)&       0.096         &       0.107         &       0.069         &       0.073         \\
Robust p-value&       0.000         &       0.898         &       0.112         &       0.003         \\


==> arxiv last/TABLE_7.tex <==
RD Estimate &      -0.168\sym{**} &      -0.187\sym{**} &      -0.028         \\
            &     (0.074)         &     (0.079)         &     (0.052)         \\
Observations&        1900         &        1900         &        1900         \\
Eff. Number of obs&         378         &         395         &         545         \\
BW Loc. Poly. (h)&       0.080         &       0.083         &       0.117         \\
Robust p-value&       0.021         &       0.015         &       0.567         \\


==> arxiv last/TABLE_8_panelA.tex <==
RD Estimate &      -0.064\sym{***}&      -0.018         &      -0.087\sym{***}&      -0.018         \\
            &     (0.024)         &     (0.013)         &     (0.030)         &     (0.019)         \\
Observations&        1303         &        1052         &         770         &        1585         \\
Eff. Number of obs&         345         &         360         &         164         &         413         \\
BW Loc. Poly. (h)&       0.101         &       0.133         &       0.083         &       0.104         \\
Robust p-value&       0.010         &       0.210         &       0.003         &       0.521         \\


==> arxiv last/TABLE_8_panelB.tex <==
RD Estimate &       0.304\sym{***}&       0.380\sym{***}&       0.490\sym{***}&       0.213\sym{**} \\
            &     (0.085)         &     (0.115)         &     (0.120)         &     (0.090)         \\
Observations&        1303         &        1052         &         770         &        1585         \\
Eff. Number of obs&         367         &         200         &         178         &         408         \\
BW Loc. Poly. (h)&       0.110         &       0.075         &       0.089         &       0.103         \\
Robust p-value&       0.005         &       0.001         &       0.000         &       0.041         \\


==> arxiv last/TABLE_9_panelA.tex <==
RD Estimate &      -0.068\sym{**} &      -0.066\sym{**} &      -0.004         &      -0.022         &      -0.011         &      -0.003         \\
            &     (0.032)         &     (0.031)         &     (0.003)         &     (0.027)         &     (0.025)         &     (0.009)         \\
Observations&        1191         &        1191         &        1191         &        1164         &        1164         &        1164         \\
Eff. Number of obs&         264         &         260         &         275         &         307         &         287         &         279         \\
BW Loc. Poly. (h)&       0.083         &       0.082         &       0.088         &       0.109         &       0.101         &       0.098         \\
Robust p-value&       0.037         &       0.041         &       0.231         &       0.580         &       0.802         &       0.730         \\


==> arxiv last/TABLE_9_panelB.tex <==
RD Estimate &      -0.061         &      -0.093         &      -0.007         &      -0.045\sym{***}&      -0.040\sym{***}&      -0.005         \\
            &     (0.098)         &     (0.089)         &     (0.005)         &     (0.016)         &     (0.015)         &     (0.004)         \\
Observations&         212         &         212         &         212         &        2143         &        2143         &        2143         \\
Eff. Number of obs&          39         &          44         &          22         &         688         &         648         &         579         \\
BW Loc. Poly. (h)&       0.069         &       0.076         &       0.052         &       0.126         &       0.119         &       0.108         \\
Robust p-value&       0.360         &       0.223         &       0.157         &       0.014         &       0.020         &       0.269         \\


==> arxiv last/TABLE_9_panelC.tex <==
RD Estimate &      -0.151\sym{*}  &      -0.144\sym{*}  &      -0.007\sym{*}  &      -0.024         &      -0.021         &      -0.003         \\
            &     (0.087)         &     (0.086)         &     (0.004)         &     (0.027)         &     (0.028)         &     (0.003)         \\
Observations&          77         &          77         &          77         &          96         &          96         &          96         \\
Eff. Number of obs&          25         &          24         &          20         &          30         &          29         &          28         \\
BW Loc. Poly. (h)&       0.095         &       0.093         &       0.065         &       0.118         &       0.117         &       0.110         \\
Robust p-value&       0.108         &       0.104         &       0.031         &       0.556         &       0.649         &       0.190         \\


==> arxiv last/TABLE_A1.tex <==
            &         (1)&         (2)&         (3)&         (4)&         (5)&         (6)&         (7)&         (8)\\
\midrule
\emph{\textbf{Conflict-related violence (pre-election term)}}&            &            &            &            &            &            &            &            \\
Killings (overall)&        1635&       2.288&       4.868&         405&       2.024&       4.010&      -1.119&       0.658\\
Very selective killings&        1635&       1.437&       2.713&         405&       1.315&       2.620&      -0.984&       0.411\\
Massacres   &        1635&       0.851&       2.721&         405&       0.709&       1.977&      -0.152&       0.354\\
Occurrence of a killing (overall)&        1635&       0.069&       0.098&         405&       0.062&       0.096&      -0.032&       0.017\\
Occurrence of a very selective killing&        1635&       0.061&       0.089&         405&       0.056&       0.088&      -0.032&       0.016\\
Occurrence of a massacre&        1635&       0.011&       0.029&         405&       0.010&       0.025&      -0.002&       0.005\\
\emph{\textbf{Armed conflict (pre-election term)}}&            &            &            &            &            &            &            &            \\
Action by guerrilla&        1635&       0.466&       0.403&         405&       0.454&       0.399&      -0.126&       0.085\\
Action by paramilitaries&        1635&       0.183&       0.271&         405&       0.177&       0.257&      -0.060&       0.052\\
Action by Nal. army&        1635&       0.414&       0.379&         405&       0.414&       0.379&      -0.163&       0.077\\
Encounter paramilitaries vs guerrilla&        1635&       0.121&       0.236&         405&       0.103&       0.219&      -0.036&       0.049\\
Encounter Nal. army vs guerrilla&        1635&       0.348&       0.375&         405&       0.338&       0.369&      -0.159&       0.073\\
Encounter Nal. army vs paramilitaries&        1635&       0.091&       0.196&         405&       0.086&       0.187&      -0.039&       0.034\\
Event of massive expulsion&        1635&       0.097&       0.212&         405&       0.102&       0.225&      -0.044&       0.050\\
\emph{\textbf{Crime (pre-election term)}}&            &            &            &            &            &            &            &            \\
Overall homicide rate&        1598&      65.045&      62.271&         391&      66.895&      64.949&      -4.990&      10.596\\
Log of hectares of coca&        1269&       1.172&       2.328&         313&       1.360&       2.506&      -0.612&       0.613\\
Log of hectares of aerial spraying on coca&        1269&       0.804&       2.157&         313&       0.960&       2.323&      -0.823&       0.627\\
\emph{\textbf{Elections (previous election)}}&            &            &            &            &            &            &            &            \\
Turnout rate&         830&       0.566&       0.115&         207&       0.571&       0.114&      -0.044&       0.024\\
Number of parties in council&        1244&       4.796&       1.992&         304&       4.740&       1.977&       0.193&       0.435\\
Council fractionalization&        1629&       0.967&       0.116&         403&       0.980&       0.088&      -0.026&       0.023\\
Liberal party in council&        1244&       0.901&       0.299&         304&       0.862&       0.346&       0.117&       0.078\\
Conservative party in council&        1244&       0.699&       0.459&         304&       0.678&       0.468&       0.054&       0.122\\
Left-wing party in council&        1244&       0.225&       0.418&         304&       0.217&       0.413&      -0.129&       0.087\\
Party with paramilitary links in council&        1244&       0.397&       0.489&         304&       0.444&       0.498&       0.027&       0.121\\
Mayor from Liberal party&        1629&       0.397&       0.489&         403&       0.390&       0.488&      -0.058&       0.112\\
Mayor from Conservative party&        1629&       0.191&       0.393&         403&       0.218&       0.414&       0.124&       0.086\\
Mayor from left-wing party&        1629&       0.022&       0.147&         403&       0.010&       0.099&       0.012&       0.029\\
Mayor from party with paramilitary links&        1629&       0.056&       0.230&         403&       0.067&       0.250&       0.075&       0.058\\
\emph{\textbf{Economy and institutions}}&            &            &            &            &            &            &            &            \\
Municipal category (first year of term)&         835&       5.819&       0.625&         208&       5.889&       0.503&       0.135&       0.141\\
\% unsatisfied basic needs (1993 or 2005)&        1635&      52.506&      21.142&         405&      52.540&      21.515&      -4.719&       4.109\\
Schools per 1000 inhab. (1997)&        1585&      34.058&      19.287&         387&      35.620&      20.070&      -4.586&       5.893\\
Hospitals per 1000 inhab. (1997)&        1585&       3.027&       2.706&         387&       3.145&       2.922&      -0.189&       0.508\\
Bank branches per 1000 inhab. in 1997&        1379&       7.510&       3.964&         331&       7.654&       3.720&       0.176&       0.738\\
Courts per 1000 inhab. (1997)&        1585&      10.095&       8.223&         388&      10.065&       8.143&       1.581&       1.416\\
Police stations per 1000 inhab. (1997)&        1581&       4.560&       2.072&         385&       4.744&       2.083&      -0.491&       0.300\\
\emph{\textbf{Fiscal outcomes (pre-election term)}}&            &            &            &            &            &            &            &            \\
Log current spending per capita&        1613&      -2.508&       0.535&         401&      -2.515&       0.588&       0.085&       0.118\\
Log fixed capital spending per capita&        1612&      -2.255&       0.568&         401&      -2.220&       0.594&      -0.027&       0.106\\
Log other capital spending per capita&        1607&      -2.206&       0.898&         401&      -2.188&       0.878&      -0.172&       0.185\\
Log tax revenue per capita&        1612&      -3.572&       1.134&         400&      -3.598&       1.113&       0.098&       0.189\\
Log royalties per capita&        1064&      -5.086&       2.614&         257&      -5.153&       2.797&      -0.078&       0.739\\
Log transfers per capita&        1591&      -1.803&       0.499&         398&      -1.785&       0.478&       0.053&       0.094\\
Total deficit per capita&        1615&      -0.015&       0.278&         401&      -0.035&       0.502&      -0.105&       0.117\\
\emph{\textbf{Geographic characteristics}}&            &            &            &            &            &            &            &            \\
Surface area (km2)&        1635&    1212.579&    3717.283&         405&    1451.821&    4693.372&    -818.574&     829.630\\
Mean altitude (m)&        1596&    1028.048&    1487.873&         390&     998.369&     918.108&      97.744&     162.835\\
Distance to Bogota (km)&        1635&     350.255&     189.249&         405&     353.554&     189.256&      -2.283&      23.116\\
Distance to the capital of department (km)&        1635&      81.685&      58.385&         405&      79.743&      57.638&      -1.267&      11.366\\
\% Municipalities on the Atlantic coast&        1635&       0.239&       0.426&         405&       0.235&       0.424&       0.015&       0.103\\
\% Municipalities in the eastern region&        1635&       0.179&       0.383&         405&       0.200&       0.400&       0.066&       0.095\\
\% Municipalities in the central region&        1635&       0.175&       0.380&         405&       0.173&       0.379&       0.006&       0.079\\
\% Municipalities on the Pacific coast&        1635&       0.202&       0.402&         405&       0.207&       0.406&      -0.064&       0.097\\
\% Municipalities in Antioquia&        1635&       0.150&       0.358&         405&       0.126&       0.332&      -0.043&       0.078\\
\% Municipalities in the Amazon region&        1635&       0.055&       0.228&         405&       0.059&       0.236&       0.008&       0.048\\


==> arxiv last/TABLE_A10_panelA.tex <==
RD Estimate &      -0.002         &      -0.070\sym{**} &      -0.005         &       0.012         \\
            &     (0.004)         &     (0.033)         &     (0.005)         &     (0.019)         \\
Observations&        2822         &        2822         &        2822         &        2817         \\
Eff. Number of obs&         855         &         656         &         755         &         563         \\
BW Loc. Poly. (h)&       0.117         &       0.091         &       0.103         &       0.078         \\
Robust p-value&       0.658         &       0.051         &       0.326         &       0.436         \\


==> arxiv last/TABLE_A10_panelB.tex <==
RD Estimate &      -2.226         &      -2.156         &      -0.070         &      -3.797         \\
            &     (1.772)         &     (1.718)         &     (0.088)         &     (3.085)         \\
Observations&        2822         &        2822         &        2822         &        2817         \\
Eff. Number of obs&         636         &         636         &         631         &         704         \\
BW Loc. Poly. (h)&       0.088         &       0.087         &       0.087         &       0.096         \\
Robust p-value&       0.239         &       0.243         &       0.402         &       0.242         \\


==> arxiv last/TABLE_A10_panelC.tex <==
RD Estimate &      -1.047         &      -1.020         &      -0.027         &      -4.420         \\
            &     (5.553)         &     (5.402)         &     (0.245)         &     (7.716)         \\
Observations&        2822         &        2822         &        2822         &        2810         \\
Eff. Number of obs&         776         &         776         &         782         &         783         \\
BW Loc. Poly. (h)&       0.106         &       0.106         &       0.107         &       0.109         \\
Robust p-value&       0.863         &       0.863         &       0.961         &       0.563         \\


==> arxiv last/TABLE_A11.tex <==
RD Estimate &       0.001         &       0.058         &       0.180         &       0.000         &       0.043         &       0.052         \\
            &     (0.002)         &     (0.067)         &     (0.194)         &     (0.003)         &     (0.067)         &     (0.206)         \\
Observations&        1900         &        1900         &        1900         &        1900         &        1900         &        1900         \\
Eff. Number of obs&         624         &         491         &         406         &         626         &         501         &         355         \\
BW Loc. Poly. (h)&       0.131         &       0.105         &       0.086         &       0.132         &       0.107         &       0.075         \\
Robust p-value&       0.400         &       0.377         &       0.341         &       0.960         &       0.481         &       0.605         \\


==> arxiv last/TABLE_A14.tex <==
RD Estimate &       0.241\sym{***}&      -0.015         &       0.196\sym{***}\\
            &     (0.078)         &     (0.075)         &     (0.074)         \\
Observations&        1900         &        1900         &        1900         \\
Eff. Number of obs&         391         &         580         &         357         \\
BW Loc. Poly. (h)&       0.083         &       0.125         &       0.076         \\
Robust p-value&       0.005         &       0.937         &       0.009         \\


==> arxiv last/TABLE_A15.tex <==
RD Estimate &      -0.152\sym{***}&      -0.154\sym{***}&      -0.035         \\
            &     (0.047)         &     (0.052)         &     (0.036)         \\
Observations&        5765         &        5765         &        5765         \\
Eff. Number of obs&         827         &         879         &        1215         \\
BW Loc. Poly. (h)&       0.058         &       0.062         &       0.086         \\
Robust p-value&       0.001         &       0.003         &       0.246         \\


==> arxiv last/TABLE_A16.tex <==
Bigger council size &      -0.040\sym{**} &      -0.000         &      -0.009         &      -0.015         &      -0.015         &      -0.051\sym{**} &       0.004         &      -0.006         &      -0.013         &      -0.013         \\
                    &     (0.017)         &     (0.015)         &     (0.015)         &     (0.020)         &     (0.018)         &     (0.021)         &     (0.017)         &     (0.018)         &     (0.025)         &     (0.023)         \\
Frenquent past violent actions&                     &       0.093\sym{***}&                     &                     &                     &                     &       0.112\sym{***}&                     &                     &                     \\
                    &                     &     (0.027)         &                     &                     &                     &                     &     (0.034)         &                     &                     &                     \\
\shortstack[l]{Bigger council size $\times$ Frenquent \\  \hspace{0.1cm}  past violent actions}&                     &      -0.076\sym{**} &                     &                     &                     &                     &      -0.112\sym{***}&                     &                     &                     \\
                    &                     &     (0.032)         &                     &                     &                     &                     &     (0.041)         &                     &                     &                     \\
Share of years with violent actions&                     &                     &       0.366\sym{***}&                     &                     &                     &                     &       0.420\sym{***}&                     &                     \\
                    &                     &                     &     (0.120)         &                     &                     &                     &                     &     (0.151)         &                     &                     \\
\shortstack[l]{Bigger council size $\times$ Share of \\ \hspace{0.1cm}  of years with violent actions}&                     &                     &      -0.398\sym{***}&                     &                     &                     &                     &      -0.523\sym{***}&                     &                     \\
                    &                     &                     &     (0.143)         &                     &                     &                     &                     &     (0.174)         &                     &                     \\
Frenquent past forced displacement&                     &                     &                     &       0.066\sym{**} &                     &                     &                     &                     &       0.085\sym{**} &                     \\
                    &                     &                     &                     &     (0.032)         &                     &                     &                     &                     &     (0.041)         &                     \\
\shortstack[l]{Bigger council size $\times$ Frenquent \\ \hspace{0.1cm}  past forced displacement}&                     &                     &                     &      -0.079\sym{*}  &                     &                     &                     &                     &      -0.121\sym{**} &                     \\
                    &                     &                     &                     &     (0.040)         &                     &                     &                     &                     &     (0.048)         &                     \\
Share of years forced displacement&                     &                     &                     &                     &       0.145\sym{***}&                     &                     &                     &                     &       0.176\sym{***}\\
                    &                     &                     &                     &                     &     (0.043)         &                     &                     &                     &                     &     (0.065)         \\
\shortstack[l]{Bigger council size $\times$ Share of \\ \hspace{0.1cm}  of years with forced displacement}&                     &                     &                     &                     &      -0.233\sym{**} &                     &                     &                     &                     &      -0.352\sym{***}\\
                    &                     &                     &                     &                     &     (0.099)         &                     &                     &                     &                     &     (0.105)         \\
R-squared           &       0.352         &       0.403         &       0.447         &       0.390         &       0.431         &       0.361         &       0.403         &       0.428         &       0.390         &       0.419         \\
Observations        &         468         &         468         &         468         &         468         &         468         &         732         &         732         &         732         &         732         &         732         \\


==> arxiv last/TABLE_A17.tex <==
RD Estimate &       0.033         &      -0.050         &      -0.134         \\
            &     (0.040)         &     (0.047)         &     (0.093)         \\
Observations&        1900         &        1900         &        1900         \\
Eff. Number of obs&         343         &         357         &         525         \\
BW Loc. Poly. (h)&       0.073         &       0.076         &       0.113         \\
Robust p-value&       0.691         &       0.287         &       0.167         \\


==> arxiv last/TABLE_A18.tex <==
paramilitary-linked mayor&      -0.011         &      -0.007         &      -0.005\sym{**} &      -0.011         &      -0.006         &      -0.005\sym{**} \\
                    &     (0.008)         &     (0.007)         &     (0.002)         &     (0.008)         &     (0.007)         &     (0.002)         \\
R-sq                &       0.714         &       0.717         &       0.509         &       0.716         &       0.719         &       0.509         \\
Observations        &        1858         &        1858         &        1858         &        1852         &        1852         &        1852         \\


==> arxiv last/TABLE_A19_panelA.tex <==
RD Estimate &       0.052\sym{**} &       0.051\sym{**} &       0.003         &       0.098         &       0.062         \\
            &     (0.022)         &     (0.021)         &     (0.003)         &     (0.085)         &     (0.074)         \\
Observations&         385         &         385         &         385         &         347         &         347         \\
Eff. Number of obs&         260         &         260         &         247         &         174         &         222         \\
BW Loc. Poly. (h)&       0.167         &       0.167         &       0.155         &       0.117         &       0.158         \\
Robust p-value&       0.020         &       0.017         &       0.297         &       0.253         &       0.375         \\


==> arxiv last/TABLE_A19_panelB.tex <==
RD Estimate &       0.030         &       0.040         &      -0.005         &       0.131         &       0.054         \\
            &     (0.026)         &     (0.026)         &     (0.004)         &     (0.104)         &     (0.059)         \\
Observations&         385         &         385         &         385         &         347         &         347         \\
Eff. Number of obs&         214         &         196         &         214         &         172         &         203         \\
BW Loc. Poly. (h)&       0.125         &       0.118         &       0.126         &       0.115         &       0.144         \\
Robust p-value&       0.222         &       0.100         &       0.278         &       0.204         &       0.381         \\


==> arxiv last/TABLE_A2.tex <==
            &         (1)&         (2)&         (3)&         (4)&         (5)&         (6)&         (7)&         (8)\\
\midrule
\emph{\textbf{Conflict-related violence (pre-election term)}}&            &            &            &            &            &            &            &            \\
Killings (overall)&         265&       7.382&      14.055&          63&       6.700&      14.036&       2.707&       3.315\\
Very selective killings&         265&       5.080&       9.006&          63&       4.149&       8.457&       2.669&       2.433\\
Massacres   &         265&       2.303&       5.862&          63&       2.550&       6.155&      -0.536&       1.412\\
Occurrence of a killing (overall)&         265&       0.180&       0.207&          63&       0.151&       0.189&       0.104&       0.077\\
Occurrence of a very selective killing&         265&       0.167&       0.196&          63&       0.136&       0.177&       0.100&       0.074\\
Occurrence of a massacre&         265&       0.031&       0.068&          63&       0.033&       0.073&       0.003&       0.015\\
\emph{\textbf{Armed conflict (pre-election term)}}&            &            &            &            &            &            &            &            \\
Action by guerrilla&         265&       0.567&       0.398&          63&       0.569&       0.411&       0.152&       0.259\\
Action by paramilitaries&         265&       0.352&       0.365&          63&       0.358&       0.346&       0.091&       0.179\\
Action by Nal. army&         265&       0.571&       0.400&          63&       0.616&       0.396&       0.059&       0.211\\
Encounter paramilitaries vs guerrilla&         265&       0.245&       0.338&          63&       0.243&       0.321&       0.155&       0.144\\
Encounter Nal. army vs guerrilla&         265&       0.452&       0.407&          63&       0.475&       0.424&       0.215&       0.256\\
Encounter Nal. army vs paramilitaries&         265&       0.275&       0.349&          63&       0.262&       0.322&       0.244&       0.171\\
Event of massive expulsion&         265&       0.119&       0.235&          63&       0.140&       0.269&      -0.103&       0.100\\
\emph{\textbf{Crime (pre-election term)}}&            &            &            &            &            &            &            &            \\
Overall homicide rate&         263&      60.375&      48.212&          63&      57.075&      60.700&       1.067&      15.722\\
Log of hectares of coca&         207&       0.678&       1.776&          55&       0.757&       1.839&       0.568&       0.456\\
Log of hectares of aerial spraying on coca&         207&       0.254&       1.040&          55&       0.191&       0.913&       0.126&       0.219\\
\emph{\textbf{Elections (previous election)}}&            &            &            &            &            &            &            &            \\
Turnout rate&         138&       0.537&       0.077&          39&       0.553&       0.085&       0.039&       0.036\\
Number of parties in council&         207&       6.749&       2.442&          55&       7.000&       1.944&       0.087&       0.576\\
Council fractionalization&         265&       0.987&       0.069&          63&       0.986&       0.083&      -0.009&       0.010\\
Liberal party in council&         207&       0.990&       0.098&          55&       0.982&       0.135&       0.020&       0.021\\
Conservative party in council&         207&       0.778&       0.417&          55&       0.655&       0.480&       0.455&       0.229\\
Left-wing party in council&         207&       0.391&       0.489&          55&       0.455&       0.503&       0.276&       0.179\\
Party with paramilitary links in council&         207&       0.551&       0.499&          55&       0.545&       0.503&       0.234&       0.277\\
Mayor from Liberal party&         265&       0.400&       0.491&          63&       0.397&       0.493&      -0.091&       0.171\\
Mayor from Conservative party&         265&       0.087&       0.282&          63&       0.048&       0.215&       0.019&       0.045\\
Mayor from left-wing party&         265&       0.064&       0.245&          63&       0.095&       0.296&       0.166&       0.198\\
Mayor from party with paramilitary links&         265&       0.072&       0.258&          63&       0.095&       0.296&      -0.003&       0.195\\
\emph{\textbf{Economy and institutions}}&            &            &            &            &            &            &            &            \\
Municipal category (first year of term)&         137&       3.073&       1.865&          39&       3.308&       1.575&       0.706&       0.667\\
\% unsatisfied basic needs (1993 or 2005)&         265&      32.266&      18.021&          63&      31.057&      17.495&      -0.562&       6.670\\
Schools per 1000 inhab. (1997)&         205&      39.799&      20.204&          50&      48.913&      20.381&      -1.489&       8.783\\
Hospitals per 1000 inhab. (1997)&         205&       1.710&       0.886&          50&       1.588&       0.962&      -0.298&       0.418\\
Bank branches per 1000 inhab. in 1997&         257&       6.999&       3.956&          60&       6.416&       3.550&       1.062&       1.963\\
Courts per 1000 inhab. (1997)&         205&       9.886&       5.026&          50&      10.128&       5.337&       1.985&       2.904\\
Police stations per 1000 inhab. (1997)&         205&       2.673&       1.949&          50&       2.701&       2.129&       0.198&       1.052\\
\emph{\textbf{Fiscal outcomes (pre-election term)}}&            &            &            &            &            &            &            &            \\
Log current spending per capita&         263&      -2.394&       0.555&          62&      -2.423&       0.486&      -0.163&       0.132\\
Log fixed capital spending per capita&         264&      -2.602&       0.594&          62&      -2.657&       0.641&       0.318&       0.258\\
Log other capital spending per capita&         264&      -2.270&       1.024&          62&      -2.188&       0.863&       0.567&       0.348\\
Log tax revenue per capita&         263&      -2.574&       0.837&          62&      -2.485&       0.741&      -0.074&       0.251\\
Log royalties per capita&         203&      -5.847&       2.388&          45&      -5.434&       1.962&       1.600&       0.879\\
Log transfers per capita&         262&      -2.061&       0.649&          62&      -2.145&       0.693&       0.296&       0.268\\
Total deficit per capita&         264&      -0.008&       0.051&          62&      -0.008&       0.040&      -0.000&       0.020\\
\emph{\textbf{Geographic characteristics}}&            &            &            &            &            &            &            &            \\
Surface area (km2)&         265&    1050.407&    1314.433&          63&     995.829&    1476.018&     -85.269&     397.161\\
Mean altitude (m)&         257&     846.459&     860.950&          60&     968.900&     945.462&     177.597&     321.918\\
Distance to Bogota (km)&         265&     362.915&     214.318&          63&     367.744&     225.071&      62.552&      59.693\\
Distance to the capital of department (km)&         265&      48.935&      63.505&          63&      48.311&      57.049&      29.449&      18.872\\
\% Municipalities on the Atlantic coast&         265&       0.272&       0.446&          63&       0.222&       0.419&      -0.135&       0.235\\
\% Municipalities in the eastern region&         265&       0.245&       0.431&          63&       0.381&       0.490&       0.181&       0.257\\
\% Municipalities in the central region&         265&       0.162&       0.369&          63&       0.032&       0.177&       0.039&       0.061\\
\% Municipalities on the Pacific coast&         265&       0.192&       0.395&          63&       0.206&       0.408&      -0.110&       0.149\\
\% Municipalities in Antioquia&         265&       0.109&       0.313&          63&       0.143&       0.353&       0.013&       0.142\\
\% Municipalities in the Amazon region&         265&       0.019&       0.136&          63&       0.016&       0.126&       0.031&       0.042\\


==> arxiv last/TABLE_A20.tex <==
RD Estimate &       0.013         &       0.024         &      -0.005         \\
            &     (0.010)         &     (0.041)         &     (0.005)         \\
Observations&        1864         &        1900         &        1004         \\
Eff. Number of obs&         506         &         414         &         349         \\
BW Loc. Poly. (h)&       0.111         &       0.088         &       0.137         \\
Robust p-value&       0.213         &       0.840         &       0.298         \\


==> arxiv last/TABLE_A21.tex <==
RD Estimate &      -0.198         &      -0.127         \\
            &     (0.437)         &     (0.353)         \\
Observations&        1900         &        1900         \\
Eff. Number of obs&         537         &         609         \\
BW Loc. Poly. (h)&       0.115         &       0.129         \\
Robust p-value&       0.688         &       0.799         \\


==> arxiv last/TABLE_A22_panelA.tex <==
RD Estimate &       0.142         &      -0.054         &       0.011         \\
            &     (0.091)         &     (0.083)         &     (0.028)         \\
Observations&        1899         &        1899         &        1899         \\
Eff. Number of obs&         420         &         478         &         423         \\
BW Loc. Poly. (h)&       0.090         &       0.102         &       0.091         \\
Robust p-value&       0.228         &       0.571         &       0.786         \\


==> arxiv last/TABLE_A22_panelB.tex <==
RD Estimate &       0.007         &       0.002         &       0.025         \\
            &     (0.052)         &     (0.032)         &     (0.093)         \\
Observations&        1900         &        1900         &        1900         \\
Eff. Number of obs&         551         &         502         &         497         \\
BW Loc. Poly. (h)&       0.119         &       0.107         &       0.106         \\
Robust p-value&       0.840         &       0.992         &       0.986         \\


==> arxiv last/TABLE_A23_panelA.tex <==
RD Estimate &       0.775         &       1.313\sym{**} \\
            &     (0.649)         &     (0.512)         \\
Observations&         927         &         973         \\
Eff. Number of obs&         242         &         140         \\
BW Loc. Poly. (h)&       0.109         &       0.059         \\
Robust p-value&       0.351         &       0.010         \\


==> arxiv last/TABLE_A23_panelB.tex <==
RD Estimate &       0.461         &       1.276\sym{***}\\
            &     (0.652)         &     (0.495)         \\
Observations&         927         &         973         \\
Eff. Number of obs&         226         &         135         \\
BW Loc. Poly. (h)&       0.102         &       0.056         \\
Robust p-value&       0.623         &       0.009         \\


==> arxiv last/TABLE_A23_panelC.tex <==
RD Estimate &      -0.035         &      -0.077\sym{**} \\
            &     (0.032)         &     (0.032)         \\
Observations&         927         &         973         \\
Eff. Number of obs&         285         &         188         \\
BW Loc. Poly. (h)&       0.127         &       0.077         \\
Robust p-value&       0.390         &       0.017         \\


==> arxiv last/TABLE_A3.tex <==
            &         (1)&         (2)&         (3)&         (4)&         (5)&         (6)&         (7)&         (8)\\
\midrule
\emph{\textbf{Conflict-related violence (pre-election term)}}&            &            &            &            &            &            &            &            \\
Killings (overall)&        1217&       1.912&       4.036&         291&       1.652&       3.302&      -1.890&       0.664\\
Very selective killings&        1217&       1.185&       2.233&         291&       0.994&       1.932&      -1.650&       0.453\\
Massacres   &        1217&       0.727&       2.354&         291&       0.658&       1.991&      -0.266&       0.430\\
Occurrence of a killing (overall)&        1217&       0.059&       0.087&         291&       0.051&       0.082&      -0.063&       0.022\\
Occurrence of a very selective killing&        1217&       0.052&       0.078&         291&       0.045&       0.074&      -0.063&       0.020\\
Occurrence of a massacre&        1217&       0.009&       0.026&         291&       0.009&       0.023&      -0.002&       0.005\\
\emph{\textbf{Armed conflict (pre-election term)}}&            &            &            &            &            &            &            &            \\
Action by guerrilla&        1217&       0.449&       0.399&         291&       0.432&       0.393&      -0.100&       0.100\\
Action by paramilitaries&        1217&       0.164&       0.253&         291&       0.153&       0.227&      -0.052&       0.060\\
Action by Nal. army&        1217&       0.393&       0.373&         291&       0.389&       0.373&      -0.172&       0.083\\
Encounter paramilitaries vs guerrilla&        1217&       0.105&       0.219&         291&       0.082&       0.182&      -0.032&       0.062\\
Encounter Nal. army vs guerrilla&        1217&       0.329&       0.366&         291&       0.317&       0.359&      -0.209&       0.099\\
Encounter Nal. army vs paramilitaries&        1217&       0.078&       0.179&         291&       0.071&       0.164&      -0.060&       0.044\\
Event of massive expulsion&        1217&       0.087&       0.195&         291&       0.092&       0.202&       0.048&       0.050\\
\emph{\textbf{Crime (pre-election term)}}&            &            &            &            &            &            &            &            \\
Overall homicide rate&        1187&      64.302&      62.060&         282&      66.732&      64.749&     -18.812&      14.018\\
Log of hectares of coca&         943&       1.168&       2.295&         227&       1.417&       2.523&       0.124&       0.715\\
Log of hectares of aerial spraying on coca&         943&       0.806&       2.130&         227&       0.986&       2.346&      -0.259&       0.717\\
\emph{\textbf{Elections (previous election)}}&            &            &            &            &            &            &            &            \\
Turnout rate&         618&       0.571&       0.119&         150&       0.572&       0.120&      -0.038&       0.032\\
Number of parties in council&         919&       4.603&       1.929&         219&       4.438&       1.860&       0.187&       0.472\\
Council fractionalization&        1212&       0.964&       0.120&         290&       0.973&       0.102&      -0.027&       0.032\\
Liberal party in council&         919&       0.879&       0.326&         219&       0.831&       0.376&       0.103&       0.145\\
Conservative party in council&         919&       0.700&       0.459&         219&       0.658&       0.476&      -0.037&       0.203\\
Left-wing party in council&         919&       0.209&       0.407&         219&       0.205&       0.405&      -0.202&       0.120\\
Party with paramilitary links in council&         919&       0.370&       0.483&         219&       0.397&       0.490&       0.123&       0.177\\
Mayor from Liberal party&        1212&       0.381&       0.486&         290&       0.369&       0.483&      -0.331&       0.150\\
Mayor from Conservative party&        1212&       0.193&       0.395&         290&       0.214&       0.411&       0.161&       0.130\\
Mayor from left-wing party&        1212&       0.023&       0.150&         290&       0.007&       0.083&       0.036&       0.024\\
Mayor from party with paramilitary links&        1212&       0.059&       0.236&         290&       0.066&       0.248&       0.205&       0.088\\
\emph{\textbf{Economy and institutions}}&            &            &            &            &            &            &            &            \\
Municipal category (first year of term)&         623&       5.934&       0.346&         151&       5.960&       0.303&       0.031&       0.173\\
\% unsatisfied basic needs (1993 or 2005)&        1217&      54.284&      20.616&         291&      54.958&      21.010&      -1.382&       5.738\\
Schools per 1000 inhab. (1997)&        1172&      32.994&      18.975&         275&      33.644&      18.870&      -8.078&       7.810\\
Hospitals per 1000 inhab. (1997)&        1172&       3.298&       3.007&         275&       3.493&       3.334&      -1.493&       0.873\\
Bank branches per 1000 inhab. in 1997&         990&       8.106&       4.046&         223&       8.429&       3.475&      -0.973&       1.128\\
Courts per 1000 inhab. (1997)&        1172&      10.076&       8.129&         276&      10.171&       8.054&       0.455&       1.659\\
Police stations per 1000 inhab. (1997)&        1168&       5.103&       1.859&         273&       5.447&       1.590&      -0.197&       0.383\\
\emph{\textbf{Fiscal outcomes (pre-election term)}}&            &            &            &            &            &            &            &            \\
Log current spending per capita&        1198&      -2.504&       0.524&         287&      -2.502&       0.564&       0.055&       0.143\\
Log fixed capital spending per capita&        1200&      -2.188&       0.566&         287&      -2.121&       0.580&      -0.048&       0.157\\
Log other capital spending per capita&        1196&      -2.158&       0.907&         287&      -2.096&       0.812&      -0.004&       0.206\\
Log tax revenue per capita&        1197&      -3.669&       1.154&         286&      -3.693&       1.123&       0.061&       0.273\\
Log royalties per capita&         757&      -4.922&       2.575&         174&      -4.901&       2.621&      -1.349&       0.966\\
Log transfers per capita&        1178&      -1.728&       0.474&         285&      -1.690&       0.453&       0.098&       0.119\\
Total deficit per capita&        1200&      -0.010&       0.154&         287&      -0.013&       0.149&       0.028&       0.025\\
\emph{\textbf{Geographic characteristics}}&            &            &            &            &            &            &            &            \\
Surface area (km2)&        1217&    1070.192&    3057.046&         291&    1257.260&    3547.250&   -1021.584&    1198.158\\
Mean altitude (m)&        1189&    1006.140&    1120.339&         281&    1018.267&     929.035&      89.235&     232.707\\
Distance to Bogota (km)&        1217&     346.772&     189.067&         291&     351.468&     191.334&      -2.885&      34.905\\
Distance to the capital of department (km)&        1217&      84.123&      60.034&         291&      83.306&      59.920&      -4.183&      15.684\\
\% Municipalities on the Atlantic coast&        1217&       0.233&       0.423&         291&       0.216&       0.413&       0.016&       0.107\\
\% Municipalities in the eastern region&        1217&       0.191&       0.393&         291&       0.213&       0.410&       0.078&       0.143\\
\% Municipalities in the central region&        1217&       0.182&       0.386&         291&       0.179&       0.384&       0.056&       0.114\\
\% Municipalities on the Pacific coast&        1217&       0.210&       0.408&         291&       0.223&       0.417&      -0.191&       0.143\\
\% Municipalities in Antioquia&        1217&       0.137&       0.344&         291&       0.113&       0.318&       0.037&       0.112\\
\% Municipalities in the Amazon region&        1217&       0.047&       0.211&         291&       0.055&       0.228&      -0.068&       0.072\\


==> arxiv last/TABLE_A4.tex <==
            &         (1)&         (2)&         (3)&         (4)&         (5)&         (6)&         (7)&         (8)\\
\midrule
\emph{\textbf{Conflict-related violence (pre-election term)}}&            &            &            &            &            &            &            &            \\
Killings (overall)&         418&       3.381&       6.614&         114&       2.973&       5.314&      -1.183&       1.159\\
Very selective killings&         418&       2.171&       3.684&         114&       2.135&       3.744&      -0.714&       0.798\\
Massacres   &         418&       1.210&       3.562&         114&       0.838&       1.943&      -0.426&       0.460\\
Occurrence of a killing (overall)&         418&       0.096&       0.121&         114&       0.090&       0.120&      -0.001&       0.032\\
Occurrence of a very selective killing&         418&       0.087&       0.112&         114&       0.083&       0.112&      -0.002&       0.030\\
Occurrence of a massacre&         418&       0.015&       0.036&         114&       0.012&       0.029&      -0.005&       0.008\\
\emph{\textbf{Armed conflict (pre-election term)}}&            &            &            &            &            &            &            &            \\
Action by guerrilla&         418&       0.516&       0.409&         114&       0.510&       0.411&      -0.237&       0.131\\
Action by paramilitaries&         418&       0.239&       0.310&         114&       0.238&       0.315&      -0.143&       0.112\\
Action by Nal. army&         418&       0.472&       0.390&         114&       0.480&       0.390&      -0.172&       0.111\\
Encounter paramilitaries vs guerrilla&         418&       0.166&       0.275&         114&       0.156&       0.288&      -0.137&       0.109\\
Encounter Nal. army vs guerrilla&         418&       0.402&       0.393&         114&       0.390&       0.389&      -0.157&       0.114\\
Encounter Nal. army vs paramilitaries&         418&       0.126&       0.236&         114&       0.126&       0.230&      -0.054&       0.066\\
Event of massive expulsion&         418&       0.126&       0.253&         114&       0.126&       0.273&      -0.203&       0.102\\
\emph{\textbf{Crime (pre-election term)}}&            &            &            &            &            &            &            &            \\
Overall homicide rate&         411&      67.191&      62.902&         109&      67.319&      65.761&      -6.892&      11.532\\
Log of hectares of coca&         326&       1.183&       2.426&          86&       1.210&       2.469&      -1.435&       0.860\\
Log of hectares of aerial spraying on coca&         326&       0.798&       2.236&          86&       0.891&       2.274&      -1.048&       0.839\\
\emph{\textbf{Elections (previous election)}}&            &            &            &            &            &            &            &            \\
Turnout rate&         212&       0.552&       0.101&          57&       0.568&       0.098&      -0.040&       0.044\\
Number of parties in council&         325&       5.342&       2.066&          85&       5.518&       2.068&      -0.102&       0.893\\
Council fractionalization&         417&       0.973&       0.104&         113&       0.998&       0.026&      -0.016&       0.015\\
Liberal party in council&         325&       0.963&       0.189&          85&       0.941&       0.237&      -0.005&       0.074\\
Conservative party in council&         325&       0.698&       0.460&          85&       0.729&       0.447&       0.087&       0.155\\
Left-wing party in council&         325&       0.271&       0.445&          85&       0.247&       0.434&      -0.022&       0.151\\
Party with paramilitary links in council&         325&       0.474&       0.500&          85&       0.565&       0.499&      -0.188&       0.154\\
Mayor from Liberal party&         417&       0.444&       0.497&         113&       0.442&       0.499&       0.282&       0.177\\
Mayor from Conservative party&         417&       0.185&       0.388&         113&       0.230&       0.423&       0.015&       0.147\\
Mayor from left-wing party&         417&       0.019&       0.137&         113&       0.018&       0.132&       0.068&       0.060\\
Mayor from party with paramilitary links&         417&       0.046&       0.209&         113&       0.071&       0.258&      -0.047&       0.102\\
\emph{\textbf{Economy and institutions}}&            &            &            &            &            &            &            &            \\
Municipal category (first year of term)&         212&       5.481&       1.019&          57&       5.702&       0.801&       0.473&       0.230\\
\% unsatisfied basic needs (1993 or 2005)&         418&      47.327&      21.815&         114&      46.366&      21.648&     -13.892&       6.296\\
Schools per 1000 inhab. (1997)&         413&      37.075&      19.860&         112&      40.472&      22.099&       3.072&       7.510\\
Hospitals per 1000 inhab. (1997)&         413&       2.256&       1.284&         112&       2.291&       1.103&       0.887&       0.341\\
Bank branches per 1000 inhab. in 1997&         389&       5.991&       3.298&         108&       6.055&       3.714&       1.857&       0.950\\
Courts per 1000 inhab. (1997)&         413&      10.151&       8.493&         112&       9.804&       8.391&       2.080&       2.599\\
Police stations per 1000 inhab. (1997)&         413&       3.025&       1.863&         112&       3.028&       2.153&      -0.581&       0.584\\
\emph{\textbf{Fiscal outcomes (pre-election term)}}&            &            &            &            &            &            &            &            \\
Log current spending per capita&         415&      -2.521&       0.568&         114&      -2.546&       0.647&       0.259&       0.212\\
Log fixed capital spending per capita&         412&      -2.452&       0.527&         114&      -2.467&       0.559&      -0.153&       0.213\\
Log other capital spending per capita&         411&      -2.345&       0.855&         114&      -2.420&       0.990&      -0.291&       0.255\\
Log tax revenue per capita&         415&      -3.291&       1.026&         114&      -3.358&       1.054&       0.400&       0.244\\
Log royalties per capita&         307&      -5.490&       2.672&          83&      -5.683&       3.083&       1.648&       1.166\\
Log transfers per capita&         413&      -2.017&       0.505&         113&      -2.026&       0.456&      -0.178&       0.128\\
Total deficit per capita&         415&      -0.029&       0.483&         114&      -0.091&       0.911&      -0.343&       0.315\\
\emph{\textbf{Geographic characteristics}}&            &            &            &            &            &            &            &            \\
Surface area (km2)&         418&    1627.135&    5163.573&         114&    1948.462&    6790.810&    -662.536&    1458.759\\
Mean altitude (m)&         407&    1092.049&    2240.245&         109&     947.073&     891.467&      48.333&     235.540\\
Distance to Bogota (km)&         418&     360.394&     189.638&         114&     358.879&     184.567&     -13.960&      41.070\\
Distance to the capital of department (km)&         418&      74.589&      52.722&         114&      70.648&      50.468&      -0.456&      17.076\\
\% Municipalities on the Atlantic coast&         418&       0.254&       0.436&         114&       0.281&       0.451&      -0.005&       0.200\\
\% Municipalities in the eastern region&         418&       0.144&       0.351&         114&       0.167&       0.374&      -0.001&       0.135\\
\% Municipalities in the central region&         418&       0.156&       0.363&         114&       0.158&       0.366&      -0.011&       0.147\\
\% Municipalities on the Pacific coast&         418&       0.179&       0.384&         114&       0.167&       0.374&       0.011&       0.157\\
\% Municipalities in Antioquia&         418&       0.189&       0.392&         114&       0.158&       0.366&      -0.149&       0.084\\
\% Municipalities in the Amazon region&         418&       0.079&       0.270&         114&       0.070&       0.257&       0.129&       0.083\\


==> arxiv last/TABLE_A5_panelA.tex <==
RD Estimate &       0.967\sym{*}  &       0.864\sym{*}  \\
            &     (0.494)         &     (0.498)         \\
Observations&        1635         &        1635         \\
Eff. Number of obs&         364         &         328         \\
BW Loc. Poly. (h)&       0.090         &       0.080         \\
Robust p-value&       0.078         &       0.104         \\


==> arxiv last/TABLE_A5_panelB.tex <==
RD Estimate &       1.076\sym{**} &       0.834\sym{*}  \\
            &     (0.506)         &     (0.477)         \\
Observations&         265         &         265         \\
Eff. Number of obs&          48         &          51         \\
BW Loc. Poly. (h)&       0.076         &       0.083         \\
Robust p-value&       0.072         &       0.212         \\


==> arxiv last/TABLE_A6_panelA.tex <==
RD Estimate &       0.035         &       0.039         &       2.146\sym{***}&       1.750\sym{**} \\
            &     (0.026)         &     (1.218)         &     (0.796)         &     (0.735)         \\
Observations&         532         &         683         &         683         &         683         \\
Eff. Number of obs&         151         &         159         &         110         &         115         \\
BW Loc. Poly. (h)&       0.111         &       0.092         &       0.059         &       0.063         \\
Robust p-value&       0.160         &       0.907         &       0.006         &       0.016         \\


==> arxiv last/TABLE_A6_panelB.tex <==
RD Estimate &       0.018         &       0.672         &       0.861\sym{*}  &       0.764\sym{*}  \\
            &     (0.032)         &     (0.859)         &     (0.463)         &     (0.459)         \\
Observations&        1350         &        1743         &        1743         &        1743         \\
Eff. Number of obs&         329         &         379         &         412         &         370         \\
BW Loc. Poly. (h)&       0.100         &       0.089         &       0.096         &       0.086         \\
Robust p-value&       0.607         &       0.593         &       0.098         &       0.118         \\


==> arxiv last/TABLE_A7.tex <==
RD Estimate &       0.816\sym{*}  \\
            &     (0.417)         \\
Observations&        1900         \\
Eff. Number of obs&         390         \\
BW Loc. Poly. (h)&       0.082         \\
Robust p-value&       0.070         \\


==> arxiv last/TABLE_A8_panelA.tex <==
RD Estimate &      -0.047\sym{***}&      -0.043\sym{***}&      -0.005         \\
            &     (0.010)         &     (0.009)         &     (0.003)         \\
Observations&        7128         &        7128         &        7128         \\
Eff. Number of obs&        2066         &        1909         &        1582         \\
BW Loc. Poly. (h)&       0.117         &       0.107         &       0.090         \\
Robust p-value&       0.000         &       0.000         &       0.094         \\


==> arxiv last/TABLE_A8_panelB.tex <==
RD Estimate &      -1.177\sym{**} &      -1.082\sym{***}&      -0.048         \\
            &     (0.493)         &     (0.298)         &     (0.219)         \\
Observations&        7128         &        7128         &        7128         \\
Eff. Number of obs&        1604         &        1552         &        2010         \\
BW Loc. Poly. (h)&       0.091         &       0.087         &       0.113         \\
Robust p-value&       0.015         &       0.001         &       0.800         \\


==> arxiv last/TABLE_A8_panelC.tex <==
RD Estimate &      -3.526\sym{**} &      -4.068\sym{***}&       0.157         \\
            &     (1.616)         &     (1.075)         &     (0.738)         \\
Observations&        7128         &        7128         &        7128         \\
Eff. Number of obs&        1567         &        1391         &        1552         \\
BW Loc. Poly. (h)&       0.088         &       0.078         &       0.087         \\
Robust p-value&       0.035         &       0.000         &       0.667         \\


==> arxiv last/TABLE_A9_panelA.tex <==
RD Estimate &      -0.061\sym{*}  &      -0.055\sym{*}  &      -0.015         \\
            &     (0.032)         &     (0.031)         &     (0.010)         \\
Observations&         683         &         683         &         683         \\
Eff. Number of obs&         221         &         203         &         152         \\
BW Loc. Poly. (h)&       0.130         &       0.121         &       0.088         \\
Robust p-value&       0.072         &       0.124         &       0.108         \\


==> arxiv last/TABLE_A9_panelB.tex <==
RD Estimate &      -0.037\sym{**} &      -0.032\sym{*}  &      -0.005         \\
            &     (0.019)         &     (0.017)         &     (0.006)         \\
Observations&        1743         &        1743         &        1743         \\
Eff. Number of obs&         537         &         551         &         411         \\
BW Loc. Poly. (h)&       0.126         &       0.128         &       0.096         \\
Robust p-value&       0.071         &       0.096         &       0.397         \\


==> arxiv last/TABLE_APOLKILLRATIO.tex <==
RD Estimate &      -0.033         &      -0.054\sym{***}&       0.013         \\
            &     (0.028)         &     (0.019)         &     (0.023)         \\
Observations&        2311         &        2311         &        2311         \\
Eff. Number of obs&         504         &         392         &         763         \\
BW Loc. Poly. (h)&       0.087         &       0.069         &       0.130         \\
Robust p-value&       0.126         &       0.005         &       0.616         \\


==> arxiv last/TABLE_C1_panelA.tex <==
RD Estimate &      -0.044\sym{***}&      -0.040\sym{***}&      -0.006         &       0.012         \\
            &     (0.016)         &     (0.015)         &     (0.004)         &     (0.021)         \\
Observations&        2323         &        2323         &        2323         &        2294         \\
Eff. Number of obs&         722         &         639         &         588         &         437         \\
BW Loc. Poly. (h)&       0.122         &       0.109         &       0.099         &       0.076         \\
Robust p-value&       0.013         &       0.018         &       0.182         &       0.419         \\


==> arxiv last/TABLE_C1_panelB.tex <==
RD Estimate &      -1.092         &      -0.923\sym{*}  &      -0.131         &      -3.679         \\
            &     (0.713)         &     (0.471)         &     (0.293)         &     (4.078)         \\
Observations&        2323         &        2323         &        2323         &        2294         \\
Eff. Number of obs&         570         &         554         &         663         &         601         \\
BW Loc. Poly. (h)&       0.096         &       0.095         &       0.113         &       0.103         \\
Robust p-value&       0.131         &       0.068         &       0.657         &       0.420         \\


==> arxiv last/TABLE_C1_panelC.tex <==
RD Estimate &      -3.153         &      -3.123\sym{*}  &      -0.091         &      -5.383         \\
            &     (2.406)         &     (1.750)         &     (1.003)         &     (9.571)         \\
Observations&        2323         &        2323         &        2323         &        2287         \\
Eff. Number of obs&         592         &         584         &         621         &         623         \\
BW Loc. Poly. (h)&       0.100         &       0.099         &       0.105         &       0.108         \\
Robust p-value&       0.204         &       0.082         &       0.946         &       0.641         \\


==> arxiv last/TABLE_conflictbaselinecontrolcrime.tex <==
RD Estimate &      -2.577         &      -2.790\sym{**} &      -0.020         \\
            &     (1.900)         &     (1.418)         &     (0.928)         \\
Observations&        2318         &        2318         &        2318         \\
Eff. Number of obs&         526         &         495         &         500         \\
BW Loc. Poly. (h)&       0.090         &       0.084         &       0.085         \\
Robust p-value&       0.215         &       0.072         &       0.917         \\

